The Inductive Bias of Flatness Regularization for Deep Matrix Factorization

Recent works on over-parameterized neural networks have shown that the stochasticity in optimizers has the implicit regularization effect of minimizing the sharpness of the loss function (in particular, the trace of its Hessian) over the family zero-loss solutions. More explicit forms of flatness regularization also empirically improve the generalization performance. However, it remains unclear why and when flatness regularization leads to better generalization. This work takes the first step toward understanding the inductive bias of the minimum trace of the Hessian solutions in an important setting: learning deep linear networks from linear measurements, also known as \emph{deep matrix factorization}. We show that for all depth greater than one, with the standard Restricted Isometry Property (RIP) on the measurements, minimizing the trace of Hessian is approximately equivalent to minimizing the Schatten 1-norm of the corresponding end-to-end matrix parameters (i.e., the product of all layer matrices), which in turn leads to better generalization. We empirically verify our theoretical findings on synthetic datasets.

==> additional_experiments.tex <==
\section{Experiments}

==> additional_related_work.tex <==
\newpage
\section{Additional Related Work}\label{sec:additional_related_work}

\paragraph{Sharpness-related Generalization Bounds.} Most existing sharpness-related generalizations depend on not only the sharpness of the training loss but also other complexity measures like a %$\ell_2$ or $\ell_1$ 
norm of the parameters or even undesirable dependence on the number of parameters~\citep{dziugaite2017computing,wei2019data,wei2019improved,foret2021sharpnessaware,norton2021diametrical}.  In contrast, our result only involves the trace of Hessian but not parameter norm or the number of parameters, \emph{e.g.}, our result holds for any (large) width of intermediate layers, $d_1,\ldots,d_{L-1}$. 

% \paragraph{Matrix Sensing with Restricted Isometry Property}

\paragraph{Implicit Bias of Gradient Descent on Matrix Factorization.} At first glance, overfitting could happen when the number of linear measurements is less than the size of the groundtruth matrix. Surprisingly, a recent line of works~\citep{gunasekar2017implicit,arora2019implicit,gissin2019implicit,li2020towards,razin2020implicit,belabbas2020implicit,jacot2021deep,razin2021implicit} has shown that GD starting from small initialization has a good implicit bias towards solutions with approximate recovery of ground truth. Notably, \citet{gunasekar2017implicit} show that for depth $2$, GD from infinitesimal initialization is implicitly biased to the minimum nuclear norm solution under commuting measurements and \citet{arora2019implicit} generalizes this results to deep matrix factorization for any depth. This is very similar to our main result that for all depth ($\ge 2$) the implicit regularization is minimizing nuclear norm, though the settings are different. Moreover, when the measurements satisfy RIP, \citet{li2017algorithmic,stoger2021small} show that GD exactly recovers the ground truth.



\paragraph{Sharpness minimization for two-layer matrix factorization:}
\citet{ding2022flat} show that the trace of Hessian implicit bias for two-layer matrix factorization is a rescaled version of the nuclear norm of the end-to-end matrix. Using this formula, they further prove that the flattest solution in this problem recovers the low-rank ground truth. However, matrix factorization with more than two layers is fundamentally more challenging compared to the depth two case; while we managed to obtain a formula for the trace of Hessian for deeper networks given a single measurement (see \Cref{thm:induced_regularizer_single_measurement}), as far as we know, one in general cannot obtain a closed-form solution for the trace of Hessian regularizer as a function of the end-to-end matrix for multiple measurements. In this work, we discover a way to bypass this hardness by showing that minimizing the trace of Hessian regularizer for a fixed end-to-end matrix approximately amounts to the nuclear norm of the end-to-end matrix, when the linear measurements satisfy the RIP property. As a cost of this approximation, we are not able to show the exact recovery of the low-rank ground truth, but only up to a certain precision.


\paragraph{Sharpness minimization in diagonal linear network:} \citet{ding2022flat}  show that the minimizer of trace of Hessianin a deep diagonal matrix factorization model with Gaussian linear measurements becomes the Schatten $2-2/L$ norm of a rescaled version of the end to end matrix. At first glance, their result might seem contradictory to our result in the RIP setup, as their implicit regularization is not always the Nuclear norm --- the sparsity regularization vanishes when $L\to\infty$. Similar results have been obtained by \citet{nacson2022implicit} for minimizing a different notion of sharpness among all interpolating solutions, the largest eigenvalue of Hessian, on the same diagonal linear models. The subtle difference is that since we consider the more standard setting without assuming the weight matrices are all diagonal, then in the calculation of the trace of Hessian of the loss we need to also differentiate the loss with respect to the non-diagonal entries, even though their values are zero, which is quite different from $\ell_p$ norm regularization. 
% This curiously shows the effect of letting nonzero non-diagonal entries for the weight matrices on the induced regularizer; the Schatten  $2-2/L$ norm changes to the nuclear norm under RIP, which can more effectively induce sparsity.
This curiously shows the complicated interplay between the geometry of the loss landscape and the implicit bias of the algorithm.

==> expectationiidgaussiancase.tex <==


\section{Expectation of $F(w)$ under iid Gaussian distribution}\label{app:iidgaussian}
\begin{lemma}[expectation of the implicit bias for the i.i.d Gaussian case]\label{lem:exp2}. 
Under the Gaussian iid assumption on $\{A_i\}_{i=1}^n$ we have
\begin{align*}
    R(W) &\coloneqq \mathbb E_{\{A_i\}_{i=1}^n} F(W)\\
    &=\sum_{i=2}^{L-1}\|W_L\dots W_{j+1}\|_F^2\|W_{j-1}\dots W_1\|_F^2 \\
    &+ d_0\|W_L\dots W_2\|_F^2 + d_L\|W_{L-1}\dots W_1\|_F^2.\numberthis\label{eq:Rdefinition}
\end{align*}
\end{lemma}

\begin{proof}
    For $j=\{2,\dots, L-1\}$, note that for the $k,\ell$ entry of the matrix $W_{j-1}\dots W_1 A_i W_L\dots W_{j+1}$ we have
    \begin{align}
        &\mathbb E \Big({{(W_{j-1}\dots W_1)}_k}^T A_i (W_L\dots W_{j+1})_\ell\Big)^2\\
        &= \|{(W_{j-1}\dots W_1)}_{k,}\|_2^2 \|(W_L\dots W_{j+1})_{,\ell}\|_2^2.\label{eq:entrywiseexp}
    \end{align}
    Summing Equation~\eqref{eq:entrywiseexp} for all $\ell \in \{1,\dots, d_j\}$ and $k \in \{1,\dots, d_{j-1}\}$:
    \begin{align*}
       &\mathbb E \|W_{j-1}\dots W_1A_iW_L\dots W_{j+1}\|_F^2\\
        &= \sum_{k=1}^{d_{j-1}}\sum_{\ell=1}^{d_{j}} \|{(W_{j-1}\dots W_1)}_{k,}\|_2^2 \|(W_L\dots W_{j+1})_{,\ell}\|_2^2\\
        & = \|W_L\dots W_{j+1}\|_F^2\|W_{j-1}\dots W_1\|_F^2.\numberthis\label{eq:avali}
    \end{align*}
    Moreover, regarding the term $\mathbb E \|A_iW_L\dots W_2\|_F^2$ note that the expected square of its $k$ and $\ell$ entry is
    \begin{align*}
        &\mathbb E ({A_i}_{k,}^T (W_L\dots W_2)_{,\ell})^2\\
        &= \|(W_L\dots W_2)_{,\ell}\|_2^2.\label{eq:avali}
    \end{align*}
    Summing this up for all $\ell \in \{1,\dots, d_1\}, k \in \{1,\dots, d_0\}$ we conclude
    \begin{align}
        \mathbb E \|A_i W_L\dots W_2\|_F^2 = d_0\|W_L\dots W_2\|_F^2.\label{eq:dovomi}
    \end{align}
    Similarly 
    \begin{align}
        \mathbb E \|W_{L-1}\dots W_1 A_i\|_F^2 = d_L \|W_{L-1}\dots W_1\|_F^2.\label{eq:sevomi}
    \end{align}
    Summing Equations~\eqref{eq:avali},~\eqref{eq:dovomi}, and~\eqref{eq:sevomi} completes the proof.
\end{proof}


==> expectationofgaussiancase.tex <==
\section{Expectation of $F(w)$ for the Gaussian rank one case}\label{app:rankonegaussianexp}
Here, we calculate the expectation of $F(w)$ when $A_i$'s follow a Gaussian rank one distribution. Indeed, the expectation turns out to be $R(W)$, the function that implicit bias concentrates around under general RIP setting.
\begin{lemma}[expectation of the implicit bias for the rank-one Gaussian distribution]\label{lem:expgaussian1}
    Under assumptions~\eqref{eq:assumptions1} for the distribution of $\{A_i\}_{i=1}^n$, the expected value of the implicit bias $F(W)$ over the randomness of $\{A_i\}_{i=1}^n$ is given by
    \begin{align*}
        R(W) &\coloneqq \mathbb E_{\{A_i\}_{i=1}^n}F(W) \\
        &= \sum_{j=2}^{L-1} \|W_{L}\dots W_{j+1}\|_F^2 \|W_{j-1}\dots W_{1}\|_F^2\\
        &+\| W_L\dots W_{2}\|_F^2 d_0 +\|W_{L-1}\dots W_1 {B_1}^{1/2}\|_F^2 d_L.\numberthis\label{eq:Rexplicitform}
    \end{align*}
\end{lemma}
\begin{proof}
    for every $i \in \{1,\dots, n\}$ and every $j \in \{2, \dots, L-1\}$:
    \begin{align*}
         \mathbb E_{A_i} \|W_{j-1}\dots W_{1} A_i W_{L}\dots W_{j+1}\|_F^2 &= \mathbb E_{x_i, y_i} \|W_{j-1}\dots W_1 x_i y_i^T W_L\dots W_{j+1}\|_F^2\\
        & = \mathbb E_{x_i, y_i} \|W_{j-1}\dots W_1 x_i\|_2^2\|y_i^TW_{L}\dots W_{j+1}\|_2^2\\
        & =\mathbb E_{x_i} \|W_{j-1}\dots W_1 x_i\|_2^2 \mathbb E_{y_i}\|y_i^TW_L\dots W_{j + 1}\|_2^2\\
        & = tr(W_{j-1}\dots W_1 {W_1}^T \dots {W_{j-1}}^T) \\ & \times tr({W_{j + 1}}^T\dots{W_L}^T W_L\dots W_{j + 1})\\
        & = \|W_{j-1}\dots W_1\|_F^2\|W_L\dots W_{j + 1}\|_F^2.\numberthis\label{eq:jgeneral}
    \end{align*}
Moreover, for $j = L$ we have
\begin{align*}
    \mathbb E_{A_i} \|W_{L-1}\dots W_{1} A_i\|_F^2
    & = \mathbb E_{x_1, y_1} \| W_{L-1}\dots W_1 x_i {y_i}^T\|_F^2\\
    & = \mathbb E_{x_L}\|W_{L-1}\dots W_1 x_i y_i^T \|_F^2\\
     & = \mathbb E_{x_i} \|W_{L-1}\dots W_1 x_i\|_2^2 \mathbb E_{y_i} \|y_i\|_2^2\\
    & = \|W_{L-1}\dots W_1\|_F^2 d_L,\numberthis\label{eq:j=L}
\end{align*}
and similarly for $j = 1$:
\begin{align}
    \mathbb E_{A_i} \|W_{L} \dots W_2 A_i\|_F^2 = 
    d_0 \|W_L\dots W_{2}\|_F^2.\label{eq:j=1}
\end{align}
Combining Equations~\eqref{eq:jgeneral},~\eqref{eq:j=1}, and~\eqref{eq:j=L} completes the proof.
\end{proof}


==> iidconcentration.tex <==

\begin{lemma}\label{lem:iidconcentration}
    With probability at least $1-\delta$, for any $W = (W_1,\dots, W_L)$:
    \begin{align*}
        |F(W) - R(W)| \leq n^{1/2}\log(dL/\delta)R(W),
    \end{align*}
    where $d = \max_{j=0}^L d_j$.
\end{lemma}
\begin{proof}
    For all $k \in \{1,\dots,d_1\}$ and $\ell \in \{1,\dots,d_L\}$, the variable $\Big((W_{j-1}\dots W_1)A_i (W_L\dots W_{j+1})_{k\ell}\Big)^2$ is subexponential with parameters 
    \begin{align*}
    &\|\Big((W_{j-1}\dots W_1)_{k,}\|^2\|\Big(W_L\dots W_{j+1}\Big)_{,\ell}\|^2,  \\
    &\|\Big((W_{j-1}\dots W_1)_{k,}\|^4\|\Big(W_L\dots W_{j+1}\Big)_{,\ell}\|^4.    
    \end{align*}
    Hence, we have the following concentration bound with probability at least $1-\delta/(L d_jd_{j-1})$ for their sum over the measurements:
    \begin{align*}
        &\Big|\sum_{i=1}^n \Big((W_{j-1}\dots W_1)_{k,}A_i (W_L\dots W_{j+1})_{,\ell}\Big)^2 \\
        &- n\|\Big((W_{j-1}\dots W_1)_{k,}\|^2\|\Big(W_L\dots W_{j+1}\Big)_{,\ell}\|^2\Big|\\
        &\leq \sqrt n \|\Big((W_{j-1}\dots W_1)_{k,}\|^2\|\Big(W_L\dots W_{j+1}\Big)_{,\ell}\|^2 \log(d_jd_{j-1}L/\delta).\numberthis\label{eq:concentration2}
    \end{align*}
    Summing this for all $k,\ell$ and applying a union bound, we have with probability at least $1-\delta$:
    \begin{align*}
        &\Big|\sum_i\|W_{j-1}\dots W_1 A_i W_L\dots W_{j+1}\|_F^2 - n\|W_{j-1}\dots W_1\|_F^2\|W_L\dots W_{j+1}\|_F^2\Big| \\
        &\leq 
        n^{1/2}\log(d_j d_{j-1}L/\delta)\|W_{j-1}\dots W_1\|_F^2\|W_L\dots W_{j+1}\|_F^2.
    \end{align*}
    Finally applying this concentration for all $1\leq j \leq L$ and a union bound on top:
    \begin{align*}
        &\Big| \sum_i \sum_{j} \|W_{j-1}\dots W_1 A_i W_L\dots W_{j+1}\|_F^2 \\
        &- n\sum_j \|W_{j-1}\dots W_1\|_F^2\|W_L\dots W_{j+1}\|_F^2\Big|\\
        &\leq n^{1/2}\log(dL/\delta)\sum_j \|W_{j-1}\dots W_1\|_F^2\|W_L\dots W_{j+1}\|_F^2,
    \end{align*}
    where $d$ is the maximum of $d_j$'s.
    Finally we need this argument with high probability for all matrices $(W_1,\dots, W_L)$. To this end, for each $1 \leq j \leq L$ we consider an $\epsilon$-covers $\mathcal C_1$ and $\mathcal C_2$ for the unit ball in $\mathbb R^{d_1}$ and $\mathbb R^{d_L}$ respectively.
    We now repeat the concentration argument in Equation~\eqref{eq:concentration2} for all pairs $\tilde x\in \mathcal C_1$ and $\tilde y\in \mathcal C_2$. Namely, we have with probability at least $1 - \delta/(L) e^{-\Omega()}$
    Now for an arbitrary rank one matrix $x y^T$, as $x/\|x\|$ has unit norm, there is a vector $\tilde x \in \mathcal C_1$ with $\|x/\|x\| - \tilde x\| \leq \epsilon$. Similarly for $y/\|y\|$ there is a vector $\tilde y \in \mathcla C_2$ with $|y/\|y\| - \tilde y| \leq \epsilon$. Now regarding the dot product of $xy^T$ to $A_j$ we can write
    \begin{align*}
        \langle xy^T, A_j\rangle &= x^T A_j y \\
        &= \|x\|\|y\| (x/\|x\|)^T A_j (y/\|y\|)\\
        &= \|x\|\|y\| \Big((x/\|x\| - \tilde x)^T A_j (y/\|y\|) \\
        &+ {\tilde x}^T A_j (y/\|y\| - \tilde y) + \tilde x^T A_j \tilde y\Big).
    \end{align*}
    Note that as the linear measurement matrix $A_j$ has iid Gaussian entries, we know with probability $1-\delta$ its spectral norm is bounded by $O(\sqrt n)$~\cite{}. Using this fact, we can bound the above terms:
    \begin{align*}
        &(x/\|x\| - \tilde x)^T A_j (y/\|y\|) \leq 
        \sqrt n \|x/\|x\| - \tilde x\| \leq \epsilon \sqrt n,\\
        &{\tilde x}^T A_j (y/\|y\| - \tilde y) \leq
        \sqrt n \|y/\|y\| - \tilde y\| \leq \epsilon \sqrt n.
    \end{align*}
    Plugging this above, we observe
    \begin{align*}
        \Big|\langle xy^T, A_j\rangle - \langle \tidle x {\tilde y}^T, A_j\rangle\Big| \lesssim \epsilon \sqrt n.
    \end{align*}
\end{proof}


==> motivation.tex <==
\section{Motivation}
%%% opening on SGD
Stochastic gradient descent and its different variants has become the conventional tool to train neural networks. Often neural nets have better precision in the overparameterized regime, when the number of parameters is picked to be larger than the number of training examples. As a result of this overparameterization, there is usually an infinite setting of the weights of the network with zero training loss; yet neural network can generalize quite well on test data. This surprising generalization behavior perhaps is tied up to the specific trajectory that SGD traverse in the training phase to reach small or zero training loss~\cite{}, which can impose an implicit bias among the set of networks with low or zero training loss. For example, even though there are many networks with zero training loss, SGD can find one which is within a set of networks with a skmall overall complexity, hence, enabling the generalization gap among the networks in that class to be bounded, given the distribution of the data. 

%%%%%%%%%% implicit bias
%%%% first some related work
Nonetheless, the exact procedure of this implicit bias has been elusive to researchers for decades. %% this part should go to related work
There has been many attempts recently on showing convergence and possibly generalization for neural networks. Neural tangent kernel is a popular idea in this regard where the network is approximated by a function in the RKHS space of a specific kernel in a specific regime of initialization. In this regime, the behavior of GD can be characterized nicely as roughly finding this minimum RKHS norm function in this space. Nonetheless, this is not the case for SGD. Plus, neural tangent kernel is unable to fully explain the full advantange of neural networks, specifically compared to kernel methods. There has been attempts to characterize certain constraints on the solution that SGD convergence to, e.g. a solution with bounded norm in case when we apply SGD on the regularized loss with the norm of the weights~\cite{}. These results exploit the ability of SGD in escaping strict saddle point. Although they provdie some insight on the implicit bias for norm regularized SGD, they cannot argue about SGD on training loss and that which network with zero training loss it converge to; specifically, the cannot argue about the trajectory of SGD before or  after reaching zero loss. 
Motivated by idea from satistical physics, another line of work tries to approximate the trajectory of SGD with a specific ODE in the space of disitributions on the neurons~\cite{}. Nonetheless, This approximation is valid only in a particular asymptotic limit where the coefficient of the noise on the gradient (e.g. a gaussian vector) is set as the square root of the step size, which is not the conventional setting that people use with SGD in practice. Furthermore, this ODE approxiamtion can only be used to argue about the SGD path until reaching zero loss, not after. Nonetheless, it is observed practically that while hovering around small or zero training loss, SGD can still change the setting of the nework weights drastically.  
%%%%%%% now the after zero loss paper
Recently, Li et al~\cite{} characterize an asymptotic description of the behavior of SGD after reaching zero loss, in the more natural setting where the coefficient behind the noise term is proportional to the step size. Specifically, given certain technical assumptions, in the limit when step size goes to zero, they show that SGD converge to a stochastic process which can be characterized fairly explicitly using a stochastic differential equation. Notably, for Label noise SGD, they show this process is a simple gradient flow with respect to the trace of the hessian of the loss function. 
Therefore, at least locally, SGD is biased toward solutions with smaller trace of hessian. The appearance of a measure on the magnitude of the eigenvalues of the hessian in particular is encouraging for researchers as experiments show that SGD often converge to regions of the loss function with low sharpness.
%%%% now motivative our problem
Given this implicit bias for label noise SGD, it is yet not clear which neural network with zero training loss has the smallest trace of hessian. In this work we take the frist steps to characterize this network in the case of linear neural networks. 


==> rankoneconcentration.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%% concentration of rank one case
The next key idea we apply is to show that $F(W)$ concentrates around $R(W)$.
\begin{lemma}\label{lem:concentration}
    With probability at least $1 - \delta$ we have for any $W = (W_1, \dots, W_L)$:
    \begin{align*}
        |F(W) - R(W)| \leq n^{-1/4}R(W) \log(1/\delta)^2.
    \end{align*}
\end{lemma}
\begin{proof}
     For sake of convenience of the proof, we define the helper variables $\tilde x_i, \tilde y_i$ such that 
     \begin{align*}
     x_i = {B_1}^{1/2}\tilde x_i, y_i = {B_2}^{1/2}\tilde y_i,    
     \end{align*}
      such that for every unit norm vector $v$, $v^T \tilde x_i$ and $v^T \tilde y_i$ are standard subgaussian.
     The key to this concentration result we show in Lemma~\ref{lem:subgaussiam} is that the fourth root of the sum $\big(\sum_{i=1}^n \|W_{j-1}\dots W_1x_i\|^2\|y_i^T W_L\dots W_{j+1}\|^2\big)^{1/4}$ is a subgaussian variable with parameter 
     \begin{align}
         \sigma^2 = \|W_{j-1}\dots W_1 {B_1}^{1/2}\|_F\|{B_2}^{1/2}W_L\dots W_{j+1}\|_F.\label{eq:sefr}
     \end{align}
    Therefore, for the variable 
        \begin{align*}
            Z = \big(\sum_{i=1}^n \|W_{j-1}\dots W_1x_i\|^2\|y_i^T W_L\dots W_{j+1}\|^2\big)^{1/4},
        \end{align*}
        we have with probability at least $1-\delta$,
        \begin{align}
            \mathbb E Z - \log^{1/2}(1/\delta)\sigma \leq Z 
            \leq \mathbb E Z + \log^{1/2}(1/\delta) \sigma.\label{eq:aval}
        \end{align}
        Also note that form Jensen
        \begin{align*}
            (\mathbb E Z)^4 &\leq \mathbb E Z^4 \\
            &=\mathbb E \sum_{i=1}^n \|W_{j-1}\dots W_1x_i\|^2\|y_i^T W_L\dots W_{j+1}\|^2\\
            &= n \|W_{j-1}\dots W_1 {B_1}^{1/2}\|_F^2\| {B_2}^{1/2} W_L\dots W_{j+1}\|_F^2.\numberthis\label{eq:dovomi}
        \end{align*}
    Combining Equations~\eqref{eq:aval} and~\eqref{eq:dovomi} and noting the definition of $\sigma$ in~\eqref{eq:sefr}, we see that with probability at least $1-\delta$
    \begin{align*}
        & (\mathbb E Z)^4 - n^{3/4}\|W_{j-1}\dots W_1 {B_1}^{1/2}\|_F^2\| {B_2}^{1/2}W_L\dots W_{j+1}\|_F^2 \log(1/\delta)^2
        \\
        & \leq Z^4 \\
        &\leq (\mathbb E Z)^4 + n^{3/4}\|W_{j-1}\dots W_1 {B_1}^{1/2}\|_F^2\| {B_2}^{1/2}W_L\dots W_{j+1}\|_F^2 \log(1/\delta)^2.\numberthis\label{eq:onej}
    \end{align*}
    But it is easy to see that Equation~\eqref{eq:onej} implies also with probability at least $1-\delta$:
    \begin{align*}
         & \mathbb E Z^4 - n^{3/4}\|W_{j-1}\dots W_1 {B_1}^{1/2}\|_F^2\| {B_2}^{1/2}W_L\dots W_{j+1}\|_F^2 \log(1/\delta)^2
        \\
        & \leq Z^4 \\
        &\leq \mathbb E Z^4 + n^{3/4}\|W_{j-1}\dots W_1 {B_1}^{1/2}\|_F^2\| {B_2}^{1/2}W_L\dots W_{j+1}\|_F^2 \log(1/\delta)^2.
    \end{align*}
    This is because the expectation of $Z^4$ should be in the same interval.
    
    Summing Equation~\eqref{eq:onej} for all $i \in \{1,\dots,n\}$ plus a union bound implies that with probability at least $1-n\delta$,
    \begin{align}
        &\big| \sum_{i=1}^n \|W_{j-1}\dots W_1x_i\|^2\|y_i^T W_L\dots W_{j+1}\|^2 \\
        &- n\|W_{j-1}\dots W_1 {B_1}^{1/2}\|_F^2\| {B_2}^{1/2} W_L\dots W_{j+1}\|_F^2 \big| \\
        & \leq n^{3/4}\log(1/\delta)^2 \|W_{j-1}\dots W_1 {B_1}^{1/2}\|_F^2\| {B_2}^{1/2} W_L\dots W_{j+1}\|_F^2.\label{eq:concentrate}
    \end{align}
    \khasha{cover arguement from here: }
    Finally we have to relax the assumption of having $W_j$'s fixed. To do so, the first idea is to work with a cover of the unit ball in the space of matrices $W$. Nonetheless, this adds a factor proportional to the dimension of the matrix, i.e. $d_i \times d_{i-1}$, to our bound which is not ideal. To improve this dependency, we try to reduce this to a cover for the space of rows and columns of the matrices. More rigorously, we consider the concentration inequality that we showed in~\eqref{eq:concentrate} for a single row of $W_{j-1}\dots W_1 {B_1}^{1/2}$ and ${B_2}^{1/2}W_L\dots W_{j+1}$. Namely, for fixed vectors $w_1 \in \mathbb R^{d_1}$, $w_2 \in \mathbb R^{d_L}$, we have with probability at least $1 - \delta$:
    \begin{align*}
        &\big| \sum_{i=1}^n |w_1^T \tilde x_i |^2 |\tilde y_i^T w_2|^2 \\
        &- n\|w_1\|^2\|w_2\|^2 \big| \\
        & \leq n^{3/4}\log(n/\delta)^2\|w_1\|^2\|w_2\|^2.\numberthis\label{eq:concentrate}
    \end{align*}
    We consider $\epsilon$-covers $\mathcal C_1$ and $\mathcal C_2$ for the unit ball in $\mathbb R^{d_1}$ and $\mathbb R^{d_L}$ respectively. It is well-known that the size of an $\epsilon$ cover for $\mathbb R^d$ grows as $(1/\epsilon)^d$. Now we apply a union bound regarding the event in Equation~\eqref{eq:concentrate} for all $\tilde w_1 \in \mathcal C_1$ and $\tilde w_2 \in \mathcal C_2$ while setting $\delta = O(\epsilon^d \delta')$ for $d = d_1 + d_L$. Hence, with probability at least $1 - O(\delta')$, for all such $\tilde w_1$ and $\tilde w_2$ in the cover:
    %for all $1\leq k \leq d_1$, $1 \leq \ell \leq d_LL$:
    \begin{align*}
        &\big| \sum_{i=1}^n |\tilde w_1^T \tilde x_i |^2 |\tilde y_i^T \tilde w_2|^2 \\
        &- n\|\tilde w_1\|^2\|\tilde w_2\|^2 \big| \\
        & \leq n^{3/4}d\log(n/(\epsilon\delta'))^2\|\tilde w_1\|^2\|\tilde w_2\|^2.\label{eq:aval}
    \end{align*}
    Moreover, with probability at least $1-O(\delta')$, we have for all $i$:
    \begin{align*}
        &\|\tilde x_i\|^2 \leq d_1\log(n/\delta'),\\
        &\|\tilde y_i\|^2 \leq  d_L\log(n/\delta').\numberthis\label{eq:dovom}
    \end{align*}
    This again follows from a simple union bound for all $x_i$ and $y_i$. Now from the property of the cover, for all $w_1$ and $w_2$ with norm at most one, there exist $\tilde w_1 \in \mathcal C_1$ and $\tilde w_2 \in \mathcal C_2$ such that
    \begin{align*}
        &\|w_1 - \tilde w_1\| \leq \epsilon,\\
        &\|w_2 - \tilde w_2\| \leq \epsilon.\numberthis\label{eq:sevom}
    \end{align*}
Note that combining Equations~\eqref{eq:sevom} and~\eqref{eq:dovom}, for $w_1$
\begin{align*}
    &\sum_{i=1}^n |w_1^T \tilde x_i |^2 |\tilde y_i^T w_2|^2 - \sum_{i=1}^n |\tilde w_1^T \tilde x_i |^2 |\tilde y_i^T \tilde w_2|^2\\
    &\lesssim \epsilon\sum_i \|\tilde x_i\|^2 \|\tilde y_i\|^2\\
    & \lesssim \epsilon  n d_1 d_L \log(n/\delta')^2.
\numberthis\label{eq:yek} 
\end{align*}
where we used the fact that $w_1, w_2$ have norm one and the bounds in Equation~\eqref{eq:dovom}. Moreover, again from the property of the cover
\begin{align}
    \big|\|w_1\|^2\|w_2\|^2 - \|\tilde w_1\|^2\|\tilde w_2\|^2 \big| \lesssim \epsilon.\label{eq:coverprecision}
\end{align}
Combining Equations~\eqref{eq:aval},~\eqref{eq:yek},~\eqref{eq:sevom}, and~\eqref{eq:coverprecision}, we have for any $w_1,w_2$ with norm at most one,
 \begin{align*}
        &\big| \sum_{i=1}^n |w_1^T \tilde x_i |^2 |\tilde y_i^T w_2|^2 \\
        &- n\| w_1\|^2\|w_2\|^2 \big| \\
        & \leq n^{3/4}(d_1+d_L)\log(n/(\epsilon\delta'))^2\|w_1\|^2\|w_2\|^2 + \epsilon  n d_1 d_L \log(n/\delta')^2.\label{eq:aval}
\end{align*}
Simply scaling both sides by an arbitrary number, we have with probability at least $1 - O(\delta')$ for any $w_1$ and $w_2$:
 \begin{align*}
        &\big| \sum_{i=1}^n |w_1^T \tilde x_i |^2 |\tilde y_i^T w_2|^2 \\
        &- n\| w_1\|^2\|w_2\|^2 \big| \\
        & \leq n^{3/4}(d_1+d_L)\log(n/(\epsilon\delta'))^2\|w_1\|^2\|w_2\|^2 \\
        & + \epsilon  n d_1 d_L \log(n/\delta')^2 \|w_1\|^2\|w_2\|^2.\label{eq:aval}
\end{align*}
    Summing this inequality for all different combinations of choices of rows of $W_{j-1}\dots W_1 {B_1}^{1/2}$ and ${B_2}^{1/2}W_L\dots W_{j+1}$ we get a concentration result for all matrices $W_1,\dots, W_L$ similar to Equation~\eqref{eq:concentrate}:
    \begin{align*}
        &\big| \sum_{i=1}^n \|W_{j-1}\dots W_1x_i\|^2\|y_i^T W_L\dots W_{j+1}\|^2 \\
        &- n\|W_{j-1}\dots W_1 {B_1}^{1/2}\|_F^2\| {B_2}^{1/2} W_L\dots W_{j+1}\|_F^2 \big| \\
        & \leq \big( n^{3/4}\big((d_1+d_L)\log(n/(\epsilon\delta'))^2 + \epsilon  n d_1 d_L \log(n/\delta')^2 \big) \\
        &\|W_{j-1}\dots W_1 {B_1}^{1/2}\|_F^2\| {B_2}^{1/2} W_L\dots W_{j+1}\|_F^2,
        \end{align*}
        with probability at least $1 - O(\delta')$. Setting $\epsilon = $
\end{proof}


    \begin{lemma}\label{lem:subgaussiam}
        Random variable $X = \big(\sum_{i=1}^n \|W_{j-1}\dots W_1x_i\|^2\|y_i^T W_L\dots W_{j+1}\|^2\big)^{1/4}$ is subGaussian with parameter $\big( \|W_{j-1}\dots W_1\|\|W_L\dots W_{j+1}\|\big)^{1/2}$. \end{lemma}
    \begin{proof}
        It is enough to show that for 
        \begin{align*}
            C^2 = \|W_{j-1}\dots W_1\|_F\|W_L\dots W_{j+1}\|_F
        \end{align*}
        we have
        \begin{align*}
            \mathbb E \exp\{X^2/C^2\} < \infty.
        \end{align*}
        Note that
        \begin{align*}
            X^2 &= \big(\sum_{i=1}^n \|W_{j-1}\dots W_1x_i\|^2\|y_i^T W_L\dots W_{j+1}\|^2\big)^{1/2}\\
            & \leq \sum_{i=1}^n \|W_{j-1}\dots W_1x_i\|\|y_i^T W_L\dots W_{j+1}\|.
        \end{align*}
        Hence, from the independence of $(x_i, y_i)$'s:
        \begin{align*}
            \mathbb E \exp\{X^2/C^2\} 
            &\leq \mathbb E \exp\{\sum_{i=1}^n \|W_{j-1}\dots W_1x_i\|\|y_i^T W_L\dots W_{j+1}\|/C^2\}\\
            &= \Pi_{i=1}^n \mathbb E \exp\{\|W_{j-1}\dots W_1x_i\|\|y_i^T W_L\dots W_{j+1}\|/C^2\}.
        \end{align*}
        But using AM-GM, for every $i$ we have
        \begin{align*}
             &\mathbb E \exp\{\|W_{j-1}\dots W_1x_i\|\|y_i^T W_L\dots W_{j+1}\|/C^2\}\\
           &\leq \mathbb E \exp\{\|W_{j-1}\dots W_1x_i\|^2/\|W_{j-1}\dots W_1\|_F^2\}\\
            & \times \mathbb E\exp\{\|y_i^T W_L\dots W_{j+1}\|/\|W_{L}\dots W_{j+1}\|_F^2\}.
        \end{align*}
        But we can bound each of these terms as
        \begin{align*}
            &\mathbb E\{\|W_{j-1}\dots W_1x_i\|^2/\|W_{j-1}\dots W_1\|_F^2\}
            \\
            & = \int_0^\infty \mathbb P(\|W_{j-1}\dots W_1x_i\|^2/\|W_{j-1}\dots W_1\|_F^2 \geq c) e^{c}dc\\
            & \leq \int \sum_{k=1}^{d_j}\mathbb P((({W_{j-1}\dots W_1)_{k,}}^T x_i)^2 / \|(W_{j-1}\dots W_1)_{k,}\|^2 \geq c) e^cdc\\
            &= \sum_k \mathbb E \exp\{(({W_{j-1}\dots W_1)_{k,}}^T x_i)^2 / \|(W_{j-1}\dots W_1)_{k,}\|^2\} < \infty,
        \end{align*}
    where the last inequality follows because for every $i$ the variable $({W_{j-1}\dots W_1)_{k,}}^T x_i$ is subexponential with parameter $\|(W_{j-1}\dots W_1)_{k,}\|^2$.
    Similarly for $y_i$'s we have
    \begin{align*}
        \mathbb E\exp\{\|y_i^T W_L\dots W_{j+1}\|/\|W_{L}\dots W_{j+1}\|_F^2\} < \infty.
    \end{align*}
    Therefore, overall implies $\mathbb E \exp\{X^2/C^2\} < \infty$ an completes the proof.
     \end{proof}
    %Using Lemma~\ref{lem:concentration}, we prove the con concentration result; for each $j$, summing variables $\|W_{j-1}\dots W_1x_i\|\|y_i^T W_L\dots W_{j+1}\|$ concentrates around its means times $n$.
    %\begin{lemma}
    % For every $1 \leq j \leq L-1$, we have with probaiblity at least $1-\delta$:
    %    \begin{align*}
    %        &\Big| \sum_{i=1}^n \|W_{j-1}\dots %W_1x_i\|^2\|y_i^T W_L\dots W_{j+1}\|^2 \\
    %        &- L\|W_{j-1}\dots %W_1\|_F^2\|W_L\dots W_{j+1}\|_F^2 \Big|\\
    %        &\leq  \log(1/\delta)^{3/2}\big( %\|W_{j-1}\dots W_1\|_F^2 \|W_L\dots %W_{j+1}\|_F^2\big)^{3/4}.
    %    \end{align*}
    %\end{lemma}
    
    
    %%%%%%%%% initial incorrect proof
    \iffalse
    First, because the variables $x_i,y_i$ are sub=Gaussian with matrices $B_1$ and $B_2$, we have with probability at least $1-\delta/n$:
    \begin{align}
        &\|x_i\|^2 \leq \log(n/\delta) tr(B_1),\\
        &\|y_i\|^2 \leq \log(n/\delta)tr(B_2).\label{eq:xiyinormbound}
    \end{align}
    Applying a union bound on top, we have with probability at least $1-\delta$, Equation~\eqref{eq:xiyinormbound} holds for all $i \in [n]$.
    
    Therefore, for any matrix $W_{L}\dots W_{j+1}$ we have with probability at least $1 - \delta$:
    \begin{align*}
        \|y_i^T W_{L}\dots W_{j+1}\|_2^2 &\leq \|y_i\|^2 \|W_{L}\dots W_{j+1}\|_F^2\\
        &\lesssim \log(n/\delta) tr(B_2) \|W_{L}\dots W_{j+1}\|_F^2.
    \end{align*}
    

    
    %Namely, for every matrix $\bar W$ with $\|\bar W\|_F = 1$
    Moreover, fpr each $1 \leq i \leq n$ and $1\leq j \leq L-1$, note that each of the random varaibles $\|W_{j-1}\dots W_1 x_i\|^2$ and $\|y_i^T W_L\dots W_{j+1}\|^2$ are subexponential with parameters $(\|W_{j-1}\dots W_1\|_F^2, \max_{1 \leq \ell \leq d_j} \|(W_{j-1}\dots W_1)_{\ell,}\|^2)$ and $(\|W_L\dots W_{j+1}\|_F^2, \max_{1 \leq \ell \leq d_j} (W_L\dots W_{j+1})_{,\ell})$.
    To make the proof clearer, given that $W_{j-1}\dots W_1$ is equal to a fixed matrix $\tilde W \in \mathbb R^{d_j \times d_1}$, we separate $\|W_{j-1}\dots W_1 x_i\|^2$ from its expectation: 
    \begin{align*}
        \|W_{j-1}\dots W_1 x_i\|^2 &= \mathbb E \|W_{j-1}\dots W_1 x_1\|^2 + \eta_{i,j}\\
        &=\|\tilde W\|_F^2 + \eta^{\tilde W}_{i,j},
    \end{align*}
    where $\eta^{\tilde W}_{i,j}$ is a sub-exponential variable with parameter $(\|\tilde W\|_F^4, \|\tilde W\|_F^2)$. Now we decompose the objective $F(W)$ as
    \begin{align*}
        F(W) &= 
        \sum_{i=1}^n \sum_{j=1}^L \|W_{j-1}\dots W_1 x_i {y_i}^T W_L \dots W_{j+1}\|_F^2\\
        &= \sum_{i=1}^n \sum_{j=1}^L \|W_{j-1}\dots W_1 x_i\|^2 \|{y_i}^T W_L \dots W_{j+1}\|^2\\
        &= \sum_i \sum_j \|W_{j-1}\dots W_1\|_F^2 \|{y_i}^T W_L \dots W_{j+1}\|^2\\
        &+\sum_i \sum_j \eta^{\tilde W}_{i,j} \|{y_i}^T W_L \dots W_{j+1}\|^2\\
        &\leq \sum_i \sum_j \|W_{j-1}\dots W_1\|_F^2 \|{y_i}^T W_L \dots W_{j+1}\|^2\\
        &+\sum_i \sum_j \eta^{\tilde W}_{i,j} \log(n/\delta)tr(B_2)\|W_L\dots W_{j+1}\|_F^2.\\
        &= \sum_i \sum_j \|W_{j-1}\dots W_1\|_F^2 \|{y_i}^T W_L \dots W_{j+1}\|^2\\
        &+ \log(n/\delta)tr(B_2) \sum_j \big(\sum_i \eta^{\tilde W}_{i,j}\big)\|W_L\dots W_{j+1}\|_F^2.
    \end{align*}
    But now for a fixed $\tilde W$, the variable $\sum_j \eta^{\tilde W}_{i,j}$ is sub-exponential with parameter 
    \begin{align*}
        n\|\tilde W\|^4.
    \end{align*}
To obtain a concentration bound independent of the choice of $\tilde W$,
we consider an $\epsilon$-cover $\mathcal C_\epsilon$ for the euclidean unit ball $\mathcal B_1 = \{\tilde w \in \mathbb R^{d_L}, \ \|\tilde w\|_2 \leq 1\}$. Namely, for every vector $w$ with $\|w\| \leq 1$, there exists a $\tilde w \in \mathcal C_\epsilon$ such that
    \begin{align*}
        \|w - \tilde w\|_2\leq \epsilon.
    \end{align*}
    Now for each
    %and has their $k$th moment bounded as
    %\begin{align*}
    %    &(\mathbb E (\|W_{j-1}\dots W_1x_i\|_2^2)^k)^{1/k} \lesssim \|W_{j-1}\dots W_1\|_F^2 k^2,\\
    %    &(\mathbb E (\|y_i^TW_{L}\dots W_{j+1}\|_2^2)^k)^{1/k} \lesssim \|W_{L}\dots W_{j+1}\|_F^2 k^2).
    %\end{align*}
\fi
%\end{proof}


==> rankoneconcentration2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%% concentration of rank one case
\section{RIP for Gaussian rank one measurements}
Here we show that when $A_i = \frac{1}{n}x_i y_i^T$ where $x_i \in \mathbb R^{d_0}, y_i \in \mathbb R^{d_L}$ are standard Gaussian vectors, then the set $\{A_i\}_{i=1}^n$ satisfies $(\delta,1)$-RIP as long as $n = \Omega(d_L d_0)$.
    
      
      Now given an arbitrary rank one matrix $w_1 w_2^T$, we want to show a concentration result for the following sum:
      \begin{align*}
          &\frac{1}{n}\sum_{i=1}^n \langle w_1 w_2^T , x_i {y_i}^T\rangle^2 =\frac{1}{n}\sum_{i=1}^n (w_1^T x_i)^2 (w_2^T y_i)^2.
      \end{align*}
      the key to this concentration result we show in Lemma~\ref{lem:subgaussiam} is that the fourth root of the sum $\big(\sum_{i=1}^n \|w_1^T x_i\|^2\|y_i^T w_2\|^2\big)^{1/4}$ is a subgaussian variable with parameter 
     \begin{align}
         \sigma^2 = \|w_1\|\|w_2\|.\label{eq:sefr}
     \end{align}
    Therefore, for the variable 
        \begin{align*}
            Z = \big(\sum_{i=1}^n \|w_1^T x_i\|^2\|y_i^T w_2\|^2\big)^{1/4},
        \end{align*}
        we have with probability at least $1-\delta$,
        \begin{align}
            \mathbb E Z - \log^{1/2}(1/\delta)\sigma \leq Z 
            \leq \mathbb E Z + \log^{1/2}(1/\delta) \sigma.\label{eq:aval}
        \end{align}
        Also note that from Jensen
        \begin{align*}
            (\mathbb E Z)^4 &\leq \mathbb E Z^4 \\
            &=\mathbb E \sum_{i=1}^n \|w_1^T x_i\|^2\|y_i^T w_2\|^2\\
            &= n \|w_1\|^2\|w_2\|^2.\numberthis\label{eq:dovomi}
        \end{align*}
    Combining Equations~\eqref{eq:aval} and~\eqref{eq:dovomi} and noting the definition of $\sigma$ in~\eqref{eq:sefr}, we see that with probability at least $1-\delta$
    \begin{align*}
        & (\mathbb E Z)^4 - n^{3/4}\|w_1\|_F^2\|w_2\|_F^2 \log(1/\delta)^2
        \\
        & \leq Z^4 \\
        &\leq (\mathbb E Z)^4 + n^{3/4}\|w_1\|_F^2\|w_2\|_F^2 \log(1/\delta)^2.\numberthis\label{eq:onej}
    \end{align*}
    But it is easy to see that Equation~\eqref{eq:onej} implies with probability at least $1-\delta$:
    \begin{align*}
         & \mathbb E Z^4 - n^{3/4}\|w_1\|^2\| w_2\|_F^2 \log(1/\delta)^2
        \\
        & \leq Z^4 \\
        &\leq \mathbb E Z^4 + n^{3/4}\|w_1\|^2\|w_2\|^2 \log(1/\delta)^2.
    \end{align*}
    This is because the expectation of $Z^4$ should be in the same interval.
    
    Summing Equation~\eqref{eq:onej} for all $i \in \{1,\dots,n\}$ plus a union bound implies that with probability at least $1-n\delta$,
    \begin{align}
        &\big| \sum_{i=1}^n \|w_1^Tx_i\|^2\|y_i^T w_2\|^2 \\
        &- n\|w_1\|_F^2\|w_2\|_F^2 \big| \\
        & \leq n^{3/4}\log(1/\delta)^2 \|w_1\|_F^2\|w_2\|_F^2.\label{eq:concentrate}
    \end{align}
    \khasha{cover argument from here: }
    Finally we have to relax the assumption of having $W_j$'s fixed. To do so, we consider a cover $\mathbb R^{d_0} \times \mathbb R^{d_L}$. More rigorously, we consider the concentration inequality that we showed in Equation~\eqref{eq:concentrate}. Namely, for fixed vectors $w_1 \in \mathbb R^{d_1}$, $w_2 \in \mathbb R^{d_L}$, we have with probability at least $1 - \delta$:
    \begin{align*}
        &\big| \sum_{i=1}^n |w_1^T \tilde x_i |^2 |\tilde y_i^T w_2|^2 \\
        &- n\|w_1\|^2\|w_2\|^2 \big| \\
        & \leq n^{3/4}\log(n/\delta)^2\|w_1\|^2\|w_2\|^2.\numberthis\label{eq:concentrate}
    \end{align*}
    Now we consider $\epsilon$-covers $\mathcal C_1$ and $\mathcal C_2$ for the unit ball in $\mathbb R^{d_0}$ and $\mathbb R^{d_L}$ respectively. It is well-known that the size of an $\epsilon$ cover for $\mathbb R^d$ grows as $(1/\epsilon)^d$. Now we apply a union bound regarding the event in Equation~\eqref{eq:concentrate} for all $\tilde w_1 \in \mathcal C_1$ and $\tilde w_2 \in \mathcal C_2$ while setting $\delta = O(\epsilon^d \delta')$ for $d = d_1 d_L$. Hence, with probability at least $1 - O(\delta')$, for all $\tilde w_1$ and $\tilde w_2$ in the cover:
    %for all $1\leq k \leq d_1$, $1 \leq \ell \leq d_LL$:
    \begin{align*}
        &\big| \sum_{i=1}^n |\tilde w_1^T \tilde x_i |^2 |\tilde y_i^T \tilde w_2|^2 \\
        &- n\|\tilde w_1\|^2\|\tilde w_2\|^2 \big| \\
        & \leq n^{3/4}d\log(n/(\epsilon\delta'))^2\|\tilde w_1\|^2\|\tilde w_2\|^2.\label{eq:aval}
    \end{align*}
    Moreover, with probability at least $1-O(\delta')$, we have for all $i$:
    \begin{align*}
        &\|\tilde x_i\|^2 \leq d_1\log(n/\delta'),\\
        &\|\tilde y_i\|^2 \leq  d_L\log(n/\delta').\numberthis\label{eq:dovom}
    \end{align*}
    This again follows from a simple union bound for all $x_i$ and $y_i$. Now from the property of the cover, for all $w_1$ and $w_2$ with norm at most one, there exist $\tilde w_1 \in \mathcal C_1$ and $\tilde w_2 \in \mathcal C_2$ such that
    \begin{align*}
        &\|w_1 - \tilde w_1\| \leq \epsilon,\\
        &\|w_2 - \tilde w_2\| \leq \epsilon.\numberthis\label{eq:sevom}
    \end{align*}
Note that combining Equations~\eqref{eq:sevom} and~\eqref{eq:dovom}, for $w_1$
\begin{align*}
    &\sum_{i=1}^n |w_1^T \tilde x_i |^2 |\tilde y_i^T w_2|^2 - \sum_{i=1}^n |\tilde w_1^T \tilde x_i |^2 |\tilde y_i^T \tilde w_2|^2\\
    &\lesssim \epsilon\sum_i \|\tilde x_i\|^2 \|\tilde y_i\|^2\\
    & \lesssim \epsilon  n d_1 d_L \log(n/\delta')^2.
\numberthis\label{eq:yek} 
\end{align*}
where we used the fact that $w_1, w_2$ have norm one and the bounds in Equation~\eqref{eq:dovom}. Moreover, again from the property of the cover
\begin{align}
    \big|\|w_1\|^2\|w_2\|^2 - \|\tilde w_1\|^2\|\tilde w_2\|^2 \big| \lesssim \epsilon.\label{eq:coverprecision}
\end{align}
Combining Equations~\eqref{eq:aval},~\eqref{eq:yek},~\eqref{eq:sevom}, and~\eqref{eq:coverprecision}, we have for any $w_1,w_2$ with norm at most one,
 \begin{align*}
        &\big| \sum_{i=1}^n |w_1^T \tilde x_i |^2 |\tilde y_i^T w_2|^2 \\
        &- n\| w_1\|^2\|w_2\|^2 \big| \\
        & \leq n^{3/4}(d_1+d_L)\log(n/(\epsilon\delta'))^2\|w_1\|^2\|w_2\|^2 + \epsilon  n d_1 d_L \log(n/\delta')^2.\label{eq:aval}
\end{align*}
Simply scaling both sides by an arbitrary number, we have with probability at least $1 - O(\delta')$ for any $w_1$ and $w_2$:
 \begin{align*}
        &\big| \sum_{i=1}^n |w_1^T \tilde x_i |^2 |\tilde y_i^T w_2|^2 \\
        &- n\| w_1\|^2\|w_2\|^2 \big| \\
        & \leq n^{3/4}(d_1+d_L)\log(n/(\epsilon\delta'))^2\|w_1\|^2\|w_2\|^2 \\
        & + \epsilon  n d_1 d_L \log(n/\delta')^2 \|w_1\|^2\|w_2\|^2.\numberthis\label{eq:aval}
\end{align*}
    Summing this inequality for all different combinations of choices of rows of $w_1$ and $w_2$ we get a concentration result for all matrices $W_1,\dots, W_L$ similar to Equation~\eqref{eq:concentrate}:
    \begin{align*}
        &\big| \sum_{i=1}^n \|w_1^T x_i\|^2\|y_i^T w_2\|^2 \\
        &- n\|w_1\|^2\|w_2\|_F^2 \big| \\
        & \leq \big( n^{3/4}\big((d_1+d_L)\log(n/(\epsilon\delta'))^2 + \epsilon  n d_1 d_L \log(n/\delta')^2 \big) \|w_1\|^2\|w_2\|_F^2,
        \end{align*}
        with probability at least $1 - O(\delta')$. Setting $\epsilon = $



    \begin{lemma}\label{lem:subgaussiam}
        For standard subgaussian vectors $x_i, y_i$, random variable $X = \big(\sum_{i=1}^n \|w_1^T x_i\|^2\|y_i^T w_2\|^2\big)^{1/4}$ is sub-Gaussian with parameter $\big( \|w\|\|w_2\|\big)^{1/2}$. \end{lemma}
        It is enough to show that for 
        \begin{align*}
            C^2 = \|w_1\|\|w_2\|
        \end{align*}
        we have
        \begin{align*}
            \mathbb E \exp\{X^2/C^2\} < \infty.
        \end{align*}
        Note that
        \begin{align*}
            X^2 &= \big(\sum_{i=1}^n (w_1^Tx_i)^2(y_i^T w_2)^2\big)^{1/2}\\
            & \leq \sum_{i=1}^n (w_1^Tx_i)(y_i^T w_2).
        \end{align*}
        Hence, from the independence of $(x_i, y_i)$'s:
        \begin{align*}
            \mathbb E \exp\{X^2/C^2\} 
            &\leq \mathbb E \exp\{\sum_{i=1}^n (w_1^T x_i)(y_i^T w_2)/C^2\}\\
            &= \Pi_{i=1}^n \mathbb E \exp\{\|w_1^Tx_i\|(y_i^T w_2)/C^2\}.
        \end{align*}
        But using AM-GM, for every $i$ we have
        \begin{align*}
             &\mathbb E \exp\{\|w_1^Tx_i\|(y_i^T w_2)/C^2\}\\
           &\leq \mathbb E \exp\{\|w_1^Tx_i\|^2/\|w_1\|^2\}\\
            & \times \mathbb E\exp\{(y_i^T w_2)/\|w_2\|_F^2\},
        \end{align*}
      and from sub-gaussianity of $w_1^T x_i$ and $w_i^T y_i$ we see that
      \begin{align*}
          &\mathbb E \exp\{\|w_1^Tx_i\|^2/\|w_1\|^2\}\leq \infty\\
          &\mathbb E\exp\{(y_i^T w_2)/\|w_2\|_F^2\}\leq \infty.
      \end{align*}
    Therefore, overall implies $\mathbb E \exp\{X^2/C^2\} < \infty$ an completes the proof.


==> twolayercase.tex <==
\section{Two layer case}

First, we consider the case where we have multiple measurements 
\begin{align*}
    tr(A_tW_e) = b_t,
\end{align*}
where 
\begin{align*}
    W_e = W_1W_2.
\end{align*}
The trace of Hessian objective becomes
\begin{align*}
    tr\nabla^2 L(W_e) = \sum_t \|W_2 A_t\|_F^2 + \|A_t W_1\|_F^2.
\end{align*}
Again, applying similar trick as the previous section, one can see that we have the following optimality condition:
\begin{align*}
    \sum_t W_2 A_t{A_t}^T {W_2}^T = \sum_t W_1^T A_t^TA_t W_1.
\end{align*}
Now writing
\begin{align*}
    \sum A_t A_t^T =  A A^T,
\end{align*}
we have
\begin{align*}
    W_2 A A^T W_2^T = W_1^T A^T A W_1.
\end{align*}
Again, considering the SVD of $W_2 A$ and $A W_1$ we see there exist orthogonal matrices $U_1, U_2, U_3$ and diagonal matrix $\Lambda$ such that
\begin{align*}
    &W_2 A = U_1 \Lambda U_2^T,\\
    &AW_1 = U_3 \Lambda U_1^T,
\end{align*}
which means
\begin{align*}
    AW_1W_2A = U_3 \Lambda^2 U_2^T.
\end{align*}
Hence, we obtain that
\begin{align*}
    tr\nabla^2 L(W_e) = \sum_t \|W_2 A_t\|_F^2 + \|A_t W_1\|_F^2. = 2\|\Lambda\|_F^2 = 2\|AW_1W_2A\|_1,
\end{align*}
where $\|.\|_1$ is the nuclear norm of the matrix.


